Generative Slate Recommendation with Reinforcement Learning

Recent research has employed reinforcement learning (RL) algorithms to optimize long-term user engagement in recommender systems, thereby avoiding common pitfalls such as user boredom and filter bubbles. They capture the sequential and interactive nature of recommendations, and thus offer a principled way to deal with long-term rewards and avoid myopic behaviors. However, RL approaches are intractable in the slate recommendation scenario - where a list of items is recommended at each interaction turn - due to the combinatorial action space. In that setting, an action corresponds to a slate that may contain any combination of items. While previous work has proposed well-chosen decompositions of actions so as to ensure tractability, these rely on restrictive and sometimes unrealistic assumptions. Instead, in this work we propose to encode slates in a continuous, low-dimensional latent space learned by a variational auto-encoder. Then, the RL agent selects continuous actions in this latent space, which are ultimately decoded into the corresponding slates. By doing so, we are able to (i) relax assumptions required by previous work, and (ii) improve the quality of the action selection by modeling full slates instead of independent items, in particular by enabling diversity. Our experiments performed on a wide array of simulated environments confirm the effectiveness of our generative modeling of slates over baselines in practical scenarios where the restrictive assumptions underlying the baselines are lifted. Our findings suggest that representation learning using generative models is a promising direction towards generalizable RL-based slate recommendation.

==> sections/3-background.tex <==
% \section{Background}
% \label{background}

% \subsection{Notations and problem definition}
% \label{problem-definition}

% We consider a slate recommendation scenario, in which a user interacts with a recommender system (RS) in a turn-by-turn manner throughout an episode of $T$ turns. At every turn $t \in \{1, \dots, T\}$, the system recommends a slate $a_t = (i_t^1, \dots, i_t^k)$ where $(i_t^j)_{1 \leqslant j \leqslant k}$ are items selected from the collection $\mathcal{I}$ and $k$ is the size of the slate set by the RS designer. The user can click on zero, one or several items in the slate and the resulting click vector $c_t = (c_t^1, \dots, c_t^k), c_t^j \in \{0, 1\}$ is returned to the RS. 

% The problem of maximizing the cumulative number of clicks throughout an episode can be modeled by a Partially Observable Markov Decision Process (POMDP) $\mathcal{M}^P = (\mathcal{S}, \mathcal{O}, \mathcal{A}, R, T, \Omega)$ defined by:
% \begin{itemize}[leftmargin=*, nosep]
%     \item A set of states $s \in \mathcal{S}$, which represent the unobservable state of the user's mind;
%     \item A set of observations $\mathcal{O}$ accessible to the system. Here observations are clicks from the previous interaction ($o_t = c_{t-1}$) and therefore lie in the space of binary vectors of size $k$: $\mathcal{O} = \{0, 1\}^k$;
%     \item A set of actions $\mathcal{A}$, which is the set of all possible slates composed of items from the collection, i.e., $|\mathcal{A}| = \frac{|\mathcal{I}|!}{(|\mathcal{I}| - k)!}$;
%     \item A reward function $R : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$, which we set here to $R(s_t,a_t) = r_t = \sum_{j=1}^k c_t^j$ in order to reflect our long-term objective of maximizing the cumulative number of clicks;
%     \item A set of unknown transition and observation probabilities, respectively $T : \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow [0,1]$ and $\Omega : \mathcal{S} \times \mathcal{A} \times \mathcal{O} \rightarrow [0,1]$, as well as a distribution over initial states $S^1 : \mathcal{S} \rightarrow [0,1]$.
% \end{itemize}
% \noindent%
% Due to the unobserved nature of the true user state in the POMDP, it is common to train agents by relying on a proxy of the state inferred from available observations. The function that provides such proxy is traditionally referred to as the \textit{belief encoder} \citep{belief}. We also define the concept of policies $\pi : \mathcal{S \times A} \rightarrow [0,1]$ and trajectories $\tau = (o_t, a_t, r_t)_{1 \leqslant t \leqslant T}$. In the remainder, we will abusively write $\tau \sim \pi$ to signify that we obtain a trajectory by first sampling an initial state $s_1$ from $S^1$ and then recursively sampling actions $T -1$ times from the policy $\pi$. The goal can now be formulated as finding an optimal policy, i.e., a policy maximizing the \emph{expected return} $\pi^* \in \mathrm{arg}\max_\pi \mathbb{E}_{\tau \sim \pi} \left[ \mathcal{R}(\tau) \right]$ with $\mathcal{R}(\tau) = \sum_{t=1}^T r_t$.

% % \subsection{Reinforcement Learning}
% % \header{General concepts} Reinforcement Learning (RL) is a learning paradigm which offers the possibility of learning policies leading to high return by reinforcing, through trial and error, the agent's estimate of the expected return %$\mathcal{R}(s,a) = \mathbb{E}_{\mathcal{M}^P, s_0 = s, a_0 = a}\left[ \sum_{t=1}^T R(s_t, a_t) \right]$ 
% % associated with each state/action pair.

% % An RL agent improves its policy $\pi$ through a succession of \emph{policy evaluation} and \emph{policy improvement} steps. While we do not wish to describe all existing methods within this work and instead refer the reader to fundamental literature \citep{sutton-barto}, we define here common concepts used in RL. The state value function $V^\pi(s) = \mathbb{E}_{\tau \sim \pi, s_1 = s}\left[ \mathcal{R}(\tau) \right]$ and the state-action value function (or simply Q-function) $Q^\pi(s,a) = \mathbb{E}_{\tau \sim \pi, s_1 = s, a_1 = a}\left[ \mathcal{R}(\tau) \right]$ describe the expected return when starting respectively in state $s$ and with the state-action couple $(s,a)$.

% % Methods based on Q-Learning \citep{q-learning} such as \citep{slateQ} evaluate directly the Q-function of the optimal policy during the policy evaluation step, and derive a policy which $\epsilon$-greedily maximizes the estimated Q-function at each timestep. Conversely, methods based on policy gradients \citep{REINFORCE} or actor-critic \citep{SAC} such as \citep{youtube-topk, IRecGAN, wolpertinger} estimate the expected return of their current policy and use gradient ascent on this return to improve their policy.
% % We provide more background about the algorithms we use in this work (REINFORCE, SAC) in the Appendices \ref{appendix:REINFORCE} and \ref{appendix:sac}.

% % \header{RL in POMDPs and belief encoder} As described in Section \ref{problem-definition}, we cannot observe the true state of the user, and we must therefore rely on proxies, i.e., observations. A common method to train agents in POMDPs is to maintain a belief about the current state \citep{belief}. Formally, we can define the set $\mathcal{B}$ of all possible belief states, i.e. all distributions $b$ over states $s \in \mathcal{S}$, and apply RL algorithms in the Belief MDP $\mathcal{M}^\mathcal{B} = (\mathcal{B}, \mathcal{A}, R^\mathcal{B}, T^\mathcal{B})$ with $ R^\mathcal{B}(b, a) = \sum_{s \in \mathcal{S}} b(s) R(s,a)$ and $T^\mathcal{B}(b, a, b') = \sum_{o \in \mathcal{O}} \mathbb{P}(b'|b,a,o) \sum_{s \in \mathcal{S}} \Omega(o | s,a) b(s)$. In practice, we assimilate $ \mathcal{B}$ to $\mathbb{R}^d, d \in \mathbb{N}$, and model $\mathbb{P}(b'|b,a,o)$ as a parameterized function $b_\psi : \mathcal{O} \times \mathcal{A} \times \mathbb{R}^d \rightarrow  \mathbb{R}^d$. We will refer to this function as the belief encoder in the remainder of the paper.

% \subsection{Assumptions made by prior work}
% \label{assumptions}

% As we briefly described in Section \ref{related-work}, previous studies \citep{youtube-topk, IRecGAN, slateQ, wolpertinger} make assumptions on the environment, i.e., user behavior, in order to make the combinatorial problem of slate recommendation tractable. In this section, we list and detail these assumptions:
% \begin{itemize}[leftmargin=*, nosep]
%     \item \textbf{Decomposable Q-value (DQ)} \citep{youtube-topk, IRecGAN, slateQ, wolpertinger}: Future rewards are caused only by clicked items, allowing to decompose the Q-values: $Q^\pi(s, a) = \sum_{i \in a} P(c_{i} |s,a) \, Q^{\text{exec}}(s, i)$ with $Q^{\text{exec}}(s, i)$ the expected future return (i.e., after the click) caused by the clicked item $i$.
%     \item \textbf{Single click (1CL)} \citep{youtube-topk, IRecGAN, slateQ}: Users can click on at most one item per slate.
%     \item \textbf{Mutual independence (MI)} \citep{youtube-topk, IRecGAN}: The returns of items in the same slate are mutually independent.\footnote{Note that the conjunction of (MI) and (1CL) as in \citep{youtube-topk, IRecGAN} is only possible when the click probability of an item in the slate does not depend on the item itself. Indeed, having dependent click probabilities (to enforce the single click) and independent items in the slate is compatible only if click probabilities do not depend on items.}
%     \item \textbf{Sequential presentation (SP)} \citep{wolpertinger}: The true click model is top-down and fading, i.e., for $l \leqslant k$ the position of item $i$ in slate $a$, $P(c^l|s, a) = P(c^l|s, a_{\leqslant l}) \leqslant P(c^l|s, \tilde{a}_{\leqslant l-1})$, where $a_{\leqslant l} = (i^1, \dots, i^{l-1}, i)$ and $\tilde{a}_{\leqslant l-1} = (i^1, \dots, i^{l-2}, i)$. Used in \citep{wolpertinger} to ensure submodularity of the Q-function.
%     \item \textbf{Knowledge of click model (CM)} \citep{slateQ}: True relevance and click probabilities are known. \citet{slateQ} leverage this assumption in order to perform planning inside this given model. Note that while (SP) constrains the user click model, (CM) also requires knowledge of its parameters, and is thus stronger.
%     \item \textbf{Execution is best (EIB)} \citep{wolpertinger}: Recommendations which are risky on the short term are never worth it, i.e., for any policies $\pi_1$, $\pi_2$, $(\mathbb{P}(R(s, \pi_1(s)) = 0) \geqslant \mathbb{P}(R(s, \pi_2(s)) = 0) \Rightarrow V^{\pi_1}(s) \leqslant V^{\pi_2}(s)) $. Note that it partly defeats the purpose of long-term optimization.
%     \item \textbf{Logged data availability (LD)} \citep{wolpertinger}: Logged data from past interactions is available. \citet{wolpertinger} require this assumption as they assume the existence of pre-trained embeddings.
% \end{itemize}
% \noindent%
% In comparison to prior work, our proposed framework has for single requirement the availability of logged data with slates and associated clicks, as we will detail in Section~\ref{method}. Note that this latter assumption is by no means restrictive as such logged data is readily available in common industrial recommendation settings.

